On the Impact of Social Media Recommendations on Opinion Consensus

We consider a discrete opinion formation problem in a setting where agents are influenced by both information diffused by their social relations and from recommendations received directly from the social media manager. We study how the "strength" of the influence of the social media and the homophily ratio affect the probability of the agents of reaching a consensus and how these factors can determine the type of consensus reached. In a simple 2-symmetric block model we prove that agents converge either to a consensus or to a persistent disagreement. In particular, we show that when the homophily ratio is large, the social media has a very low capacity of determining the outcome of the opinion dynamics. On the other hand, when the homophily ratio is low, the social media influence can have an important role on the dynamics, either by making harder to reach a consensus or inducing it on extreme opinions. Finally, in order to extend our analysis to more general and realistic settings we give some experimental evidences that our results still hold on general networks.

==> exp.tex <==
\section{Remaining Experiments}
\label{apx:exp}
Results in Section~\ref{sec3} show that convergence to consensus is affected by the initial opinions of agents: indeed conditions for non-consensus in case both initial opinions are larger than $\lambda$ in absolute value are stricter than in the case of a single initial opinion far from $0$, and the latter are much more stricter in the case of both initial opinion are close to zero. This behaviour still holds even in more complex graph structures. Specifically, Figure~\ref{fig3} shows that the consensus probability decreases as the average opinion of agents in a component goes to $1$.
\begin{figure}[htb]
  \begin{subfigure}[t]{0.49\textwidth}
\centering
\includegraphics[scale=0.415]{/ConseusProbabilityInitialMeanOpinion/BlockModel}
\caption{Two Block Model}
\label{fig3a}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
\includegraphics[scale=0.415]{/ConseusProbabilityInitialMeanOpinion/facebook}
\caption{\texttt{ego-facebook}}
\label{fig3b}
\end{subfigure}
 \caption{In Figure~\ref{fig3a} we show how the consensus probability changes when $\delta = 0.25$, $\pout = 0.2$, $\pin = 0.4$, and $b$ is set to have $\tb = 1.2\cdot\tau_1(h)$.
 %
 In Figure~\ref{fig3b} we show how the consensus probability changes when $\delta = 0.25$, $\win = 1$, $\wout$ is drawn at each simulation uniformly at random in $[0.3, 4]$, and $b$ is set to have $\tb = 1.2\cdot\tau_1(h)$.\\
 %
 Note that in this experiment the initial opinions are still drawn uniformly at random in intervals $[l_L, h_L]$ and $[l_R, h_R]$, but these interval are fixed (they are chosen to be the same interval but with opposite sign) to have that the average opinions of agents in each component has absolute value $x\delta$, with $x \in \{0, 0.6, 0.8, 1, 1.5, 2,3, 4\}$.\\
 %
The confidence intervals are shown as error bars. Similar results have been obtained for the other network models.}
\label{fig3}
\end{figure}
Interestingly, the figure highlights that a sharp change of probability occurs exactly around $\lambda=0.5$, by confirming our findings.

Actually, we run also experiments in which we impose initial opinions to be larger or smaller than $\lambda$. Again, we observe that the behaviour on complex networks is very close to the one described for the simple symmetric two-block model.
Specifically, we first considered the case in which initial opinions are restricted to be larger than $\lambda$. Figure~\ref{fig4} shows how the probability of consensus changes as $\tb$ increase in this setting.
\begin{figure}[htb]
\begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/LambdaImpossible/BlockModel}
\caption{Two Block Model}
\label{fig4a}
\end{subfigure}%
\begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/LambdaImpossible/facebook}
\caption{\texttt{ego-facebook}}
\label{fig4b}
\end{subfigure}
\caption{In Figure~\ref{fig4a} we show how the consensus probability changes when $\delta = 0.25$, $\pout = 0.2$, $\pin = 0.4$, and $b$ is set to have $\tb \in \{0.4, 0.405, 0.41, \ldots, 10\}$.\\
 %
 In Figure~\ref{fig4b} we show how the consensus probability changes when $\delta = 0.25$, $\win = \wout = 1$, and $b$ is set to have $\tb \in \{0.5, 1.5, \ldots, 10.5\}$.\\
 %
 In order to have large divergent initial opinion, these are drawn uniformly at random in intervals $[-1, -\lambda-\delta]$ and $[\lambda+\delta, 1]$.\\
 %
The confidence intervals are shown as error bars. Similar experiments have been run also on the remaining network models with very similar results.}
\label{fig4}
\end{figure}
We observe that the figure shows that the decrement of the probability of consensus occurs as soon as the value of $\tb$ is around $\tau_1(h)$. Hence, not only the general behaviour that emerges from the symmetric two-block model extends to more general networks, but we have also that the given thresholds turn out to be quite precise in describing the behaviour also in more general networks.

Similar observations hold when we consider that agents are allowed to take opinion smaller than $\lambda$ in absolute values (see Figure~\ref{fig5}).
\begin{figure}[htb]
 \begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/ZeroPossible/BlockModel}
\caption{Two Block Model}
\label{fig5a}
\end{subfigure}
\hfill
\begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/ZeroPossible/facebook}
\caption{\texttt{ego-facebook}}
\label{fig5b}
\end{subfigure}
 \caption{Figures show the results of experiments in the same settings as Figure~\ref{fig4}, except that initial opinion are not constrained to be far from zero (i.e., they are generated as described above).\\
 %
The confidence intervals are shown as error bars. Similar experiments have been run also on the remaining network models with very similar results.}
\label{fig5}
\end{figure}
Here, there are three possible phases: when $\tb$ is small, we have high probability of consensus; for intermediate values, the probability is smaller, but still far away from zero; finally, for large $\tb$, the probability of consensus get close to zero. Interestingly, the phases changes occurs, as indicated by results above, around $\tau_1(h)$ and $\tau_2(h)$.

Finally, we consider the case in which initial opinions do not diverge.
Specifically, Figure~\ref{fig6} shows that, except for real datasets, it is possible to distinguish two phases: for low values of $\tb$, there is an high probability of consensus, whereas for larger values this probability decreases (but it does not go to zero).
Moreover, Figure~\ref{fig6} confirms that the smaller is the homophily ratio the smaller $\tb$ need to be to make the probability of consensus large by allowing consensus on an opinion different from $-1, 0, 1$, as observed in Theorem~\ref{thm:conv_small}.
Interestingly, for real datasets this behaviour is not confirmed, since the probability of consensus is close to $1$ regardless the values of $\tb$ and $h$. We conjecture that this different behaviour depends on the large density of these networks with respect to the remaining ones. However, this will requires a more careful analysis that would focus on the link between the impact of social media recommendations and the structural and topological properties of the network.
\begin{figure}[htb]
 \begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/NotDivergentOpinion/BlockModel}
\caption{Two Block Model}
\label{fig6a}
\end{subfigure}
\hfill
\begin{subfigure}[c]{0.49\textwidth}
\includegraphics[scale=0.415]{/NotDivergentOpinion/random}
\caption{Random Graphs}
\label{fig6b}
\end{subfigure}\\
\begin{subfigure}[c]{\textwidth}
\centering
\includegraphics[scale=0.415]{/NotDivergentOpinion/facebook}
\caption{\texttt{ego-facebook}}
\label{fig6c}
\end{subfigure}
 \caption{In Figure~\ref{fig6a} we show the results in the same setting as Figure~\ref{fig2a}.\\
In Figure~\ref{fig6b} we show how the consensus probability changes when $\delta = 0.125$, $\wout = 1, \win \in \{0.5,1,2,4\}$ and $b$ is set to have $\tb \in \{0.5,1.5,\ldots,10.5\}$. As Figure\ref{fig2}, $h$ is the expected value of the homophily ratio over all runs involving the same value of $\win$.\\
In Figure~\ref{fig6c} we show the results in the same setting as Figure~\ref{fig2b}.\\
Note that in this experiment the initial opinions are not constrained to diverge; indeed, they are still drawn uniformly at random in intervals $[l_L,h_L]$ and $[l_R, h_R]$, but both intervals are equal to $[-1,1]$.\\
%
The confidence intervals are shown as error bars. Similar experiments have been run also on the remaining network models with very similar results.
}
\label{fig6}
\end{figure}
However, differently from what happens for the case of divergent initial opinions, we here highlight a difference between experimental and theoretical results. The latter ones show that the thresholds among the two phases should depend on the homophily ratio $h$. However, this dependence does not appear in experiments. We leave open the problem of investigating about the reasons behind this discrepancy.
% ({\color{red}{dall'analisi teorica vediamo che inizialmente dovremmo avere una consens probability bassa fino a $\tau_4$ quando $h$ è sufficientemente alto da rendere $\tau_4$ diverso da zero. Più $\delta$ è basso più questo valore di $h$ dovrebbe essere alto. Durante gli esperimenti invece abbiamo osservato che, per qualunque tipo di rete, il valore di $h$ tale per cui ho che per valori bassi di $\tb$ probabilità di consenso vicino a zero non dipende da $\delta$.}})


==> sn-article-template/sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


